Secure-by-Construction Synthesis of Cyber-Physical Systems

Correct-by-construction synthesis is a cornerstone of the confluence of formal methods and control theory towards designing safety-critical systems. Instead of following the time-tested, albeit laborious (re)design-verify-validate loop, correct-by-construction methodology advocates the use of continual refinements of formal requirements -- connected by chains of formal proofs -- to build a system that assures the correctness by design. A remarkable progress has been made in scaling the scope of applicability of correct-by-construction synthesis -- with a focus on cyber-physical systems that tie discrete-event control with continuous environment -- to enlarge control systems by combining symbolic approaches with principled state-space reduction techniques. Unfortunately, in the security-critical control systems, the security properties are verified ex post facto the design process in a way that undermines the correct-by-construction paradigm. We posit that, to truly realize the dream of correct-by-construction synthesis for security-critical systems, security considerations must take center-stage with the safety considerations. Moreover, catalyzed by the recent progress on the opacity sub-classes of security properties and the notion of hyperproperties capable of combining security with safety properties, we believe that the time is ripe for the research community to holistically target the challenge of secure-by-construction synthesis. This paper details our vision by highlighting the recent progress and open challenges that may serve as bricks for providing a solid foundation for secure-by-construction synthesis of cyber-physical systems.

==> 4_Verification/Finite_Systems/Verifying_Approximate_Opacity.tex <==

In order to verify $\delta$-approximate initial-state opacity, we construct a new system called the \emph{$\delta$-approximate initial-state estimator} defined  as follows.
\begin{definition}
Let $S=(X,X_0,X_S,U,\rTo,Y,H)$ be a metric system, with the metric $\mathbf{d}$ defined over the output set, and a constant $\delta\geq 0$.
The $\delta$-approximate initial-state estimator is a system (without outputs)
\[
S_I=(X_I,X_{I0},U,\rTo_I),
\]
where
\begin{itemize}
  \item
  $X_I\subseteq X\times 2^X$ is the set of states;
  \item
  $X_{I0}=\{(x,q)\!\in\! X\times 2^X:   x'\!\in\! q\Leftrightarrow \mathbf{d}(H(x),H(x'))\leq \delta   \}$ is the set of initial states;
  \item
  $U$ is the set of inputs, which is the same as the one in $S$;
  \item
  $\rTo_I\subseteq X_I\times U\times X_I$ is the transition function defined by:
  for any $(x,q),(x',q')\in X\times 2^X$ and $u\in U$,   $(x,q)\rTo^{u}_I(x',q')$ if
  \begin{enumerate}
  \item
  $(x',u,x)\in \rTo$; and
  \item
  $q' \!=\! \cup_{\hat{u}\in U} \mathbf{Pre}_{\hat{u}}(q) \cap \{x''\!\in\! X:   \mathbf{d}(H(x'),H(x''))\!\leq \!\delta  \}$.
  \end{enumerate}
\end{itemize}
For the sake of simplicity, we only consider the part of $S_I$ that is reachable from initial states.
\end{definition}

Intuitively, the $\delta$-approximate initial-state estimator works as follows.
Each initial state of $S_I$ is a pair consisting of a system state and its $\delta$-closed states; we consider all each pairs as the set of initial states.
Then from each state, we track \emph{backwards} states that are consistent with the output information recursively.
 Our construction is motivated by the reversed-automaton-based initial-state-estimator proposed in \cite{Wu2013ComparativeAnalysisOpacity}
 but with the following differences.
 First, the way we defined information-consistency is different. Here we treat states whose output are $\delta$-close to each other as consistent states.
 Moreover, the structure in  
 \cite{Wu2013ComparativeAnalysisOpacity}
 only requires a state space of $2^X$, while our state space is $X\times 2^X$.
The additional first component can be understood as the ``reference trajectory"  that is used to determine what is ``$\delta$-close" at each instant.
We use the following result to show the main property of  $S_I$.

The next theorem provides one of the main results of this section on the verification of $\delta$-approximate initial-state opacity of finite metric systems.

\begin{theorem}\label{thm:int}
Let $S=(X,X_0,X_S,U,\rTo_I,Y,H)$ be a finite metric system, with the metric $\mathbf{d}$ defined over the output set, and a constant $\delta\geq 0$.
Let $S_I=(X_I,X_{I0},U,\rTo_I)$ be its $\delta$-approximate initial-state estimator.
Then, $S$ is $\delta$-approximate initial-state opaque if and only if
$\forall(x,q)\in X_I: x\in X_0\cap X_S \Rightarrow q\cap X_0 \not\subseteq X_S$.
\end{theorem}

\begin{example}
\begin{figure}
  \centering
  \subfigure[$S_{I}$ when $\delta=0.1$]{\label{fig:2}
    \includegraphics[width=0.475\textwidth]{Figure/Figure2.pdf}}
  \subfigure[$S_{I}$ when $\delta=0.15$]{\label{fig:3}
    \includegraphics[width=0.475\textwidth]{Figure/Figure3.pdf}}
          \caption{Examples of $\delta$-approximate initial-state estimators.} \label{exmaple2}
\end{figure}

Let us still consider system $S$ shown in Figure~\ref{fig:1}.
The $\delta$-approximate initial-state estimator $S_I$ when $\delta=0.1$ is shown in Figure~\ref{fig:2}.
For example, for initial state $(D,\{D\})$, we have $(D,\{D\})\rTo_{I}^u (B,\{B,C\})$ since
$B\rTo^u D$ and
$\{B,C\}=  \mathbf{Pre}_{u}(\{D\}) \cap \{x\in X:   \mathbf{d}(0.1,H(x))\leq 0.1 \}
= \{B,C\}\cap\{A,B,C\}$.
However, for state $(B,\{B,C\})\in X_I$, we have $B\in X_0\cap X_S$ and $\{B,C\}\cap X_0=\{B\}\subseteq X_S$.
Therefore, by Theorem~\ref{thm:int}, we know that the system is not $0.1$-approximate initial-state opaque.
Similarly, we can also construct $S_I$ for the case of $\delta=0.15$, which is shown in Figure~\ref{fig:3}.
Since for state $(B,\{A,B,C\})\in X_I$,
which is the only state whose first component is in $X_0\cap X_S$,
we have $\{A,B,C\}\cap X_0=\{A,B\}\not\subseteq X_S$.
By Theorem~\ref{thm:int}, we know that the system is $0.15$-approximate initial-state opaque.
\end{example}

In order to verify $\delta$-approximate current-state opacity,
we can construct a new system called the \emph{$\delta$-approximate current-state estimator} in a similar way as shown in [Yin Tac].

The construction of $S_C$ is similar to $S_I$.
However, we need to track all forward runs from each pair of initial-state and its information-consistent states.
Still, we need the first component as the ``reference state" to determine what are ``$\delta$-close" states.
We use the following result to state the main properties of $S_C$.



Finally,   we can combine the $\delta$-approximate initial-state estimator $S_I$ and the $\delta$-approximate current-state estimator $S_C$ to verify $\delta$-approximate infinite-step opacity of finite metric systems.




\begin{remark}
We conclude this subsection by discussing the complexity of verifying approximate opacity.
Let $S=(X,X_0,X_S,U,\rTo,Y,H)$ be a finite metric system.
The complexity of the verification algorithms for both approximate initial-state and current-state opacity is
$O(\vert U\vert\times \vert X\vert\times2^{\vert X\vert})$, which is the size of $S_I$ or $S_C$.
For approximate infinite-step opacity, we need to construct both $S_I$ and $S_C$, and compare each pair of states in  $S_I$ and $S_C$.
Therefore, the complexity for verifying approximate infinite-step opacity using Theorem~\ref{thm:inf-veri} is
$O(\vert U\vert\times \vert X\vert^2 \times 4^{\vert X\vert})$.
It is worth noting that the complexity of verifying exact opacity  is already known to be PSPACE-complete \cite{cassez2012synthesis}. 
Using a similar reduction, we can conclude that the complexity of verifying approximate opacity as in Definition~\ref{def:opa-app}  is also PSPACE-complete for $\delta>0$. 
Finally, we note that the exponential complexity essentially comes from the subset construction to handle information uncertainty. 
In practice, the  subset construction usually results in a quite small structure; see, e.g.,  \cite{clavijo2017empirical} for detailed empirical studies on this issue. 
\end{remark}
